Zombie-Lending in the United States -- Prevalence versus Relevance

Extraordinary fiscal and monetary interventions in response to the COVID-19 pandemic have revived concerns about zombie prevalence in advanced economies. Within a sample of publicly listed U.S. companies, we find zombie prevalence and zombie-lending not to be a widespread phenomenon per se. Nevertheless, our results reveal negative spillovers of zombie-lending on productivity, capital-growth, and employment-growth of non-zombies as well as on overall business dynamism. It is predominantly the class of healthy small- and medium-sized companies that is sensitive to zombie-lending activities, with financial constraints further amplifying these effects.

==> 10_Estimation/EMPgr_Z_v3_oldEMP.tex <==
\begin{table}[h!]
%\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.75}
    \begin{center}
    %\vspace{-2cm}
    \captionsetup{justification=centering}
    \footnotesize
\caption{\label{tab:EMPgr_Z_v3} Regressions Results: Employment Growth \& Zombie-Lending \\ Zombie-Definition $Z^{NAR}$}
 

\begin{tabular}{l cccc} \hline
\addlinespace[2pt]
 Maturity ($m$) & & 1Q  $\leq m \leq$ 4Q & 1Q  $\leq m \leq$ 4Q 
 & 1Q  $\leq m \leq$ 4Q \\
 \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
 & & (1)  & (2) & (3) \\
Variables & & $\Delta EMP_{i,t}$ & $\Delta EMP_{i,t}$ & 
$\Delta EMP_{i,t}$  \\  \addlinespace[2pt] \hline

\addlinespace[10pt]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$ NZ_{i,t-1} $ & &
1.821 & 2.692 & 4.579*** \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addlinespace[5pt]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$ NZ_{i,t-1} \times SM_{i,t-1}$ & &
7.047*** & & \\ \addlinespace[5pt]

$ NZ_{i,t-1} \times SM_{i,t-1} \times \Delta log \left(BC^Z_{s,t}\right)$ & &
-0.238** & & \\ \addlinespace[5pt]

$ NZ_{i,t-1} \times SM_{i,t-1}  \times \Delta log \left(BN^Z_{s,t}\right) $& & 
-0.028 & & \\ \addlinespace[5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addlinespace[5pt]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$ NZ_{i,t-1} \times SM_{i,t-1} \times bank.dep_{i}$ & &
 & 6.843*** & \\ \addlinespace[5pt]
 
$ NZ_{i,t-1} \times SM_{i,t-1} \times bond.dep_{i}$ & &
 & 6.505*** & \\ \addlinespace[5pt] 

$ NZ_{i,t-1} \times SM_{i,t-1} \times bank.dep_{i} \times \Delta log \left(BC^Z_{s,t}\right)$ & &
 & -0.239 & \\ \addlinespace[5pt]
 
$ NZ_{i,t-1} \times SM_{i,t-1} \times bond.dep_{i} \times \Delta log \left(BN^Z_{s,t}\right)$ & &
 & -0.055 & \\ \addlinespace[5pt] 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addlinespace[5pt]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$ NZ_{i,t-1} \times SM_{i,t-1} \times bank.dep_{i}  \times no.bond_{i}$ & &
 & & 7.959*** \\ \addlinespace[5pt]

$ NZ_{i,t-1} \times SM_{i,t-1} \times bond.dep_{i}$ & & 
 & & 5.377** \\ \addlinespace[5pt]
 
$ NZ_{i,t} \times SM_{i,t-1} \times bank.dep_{i}  \times no.bond_{i} \times \Delta log \left(BC^Z_{s,t}\right)$ & &
 & & -2.996 \\ \addlinespace[5pt]

$ NZ_{i,t-1} \times SM_{i,t-1} \times bond.dep_{i} \times \Delta log \left(BN^Z_{s,t}\right)$ & & 
 & & -0.054 \\ \addlinespace[5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% $ NZ_{i,t-1} \times \Delta log\left(BC^Z_{i,t}\right) \times SM_{i,t-1} \times bank.dep_{i}  \times no.bond_{i}$ & &
% & & & & & -- \\ \addlinespace[5pt]
 
% $ NZ_{i,t-1} \times \Delta log\left(BC^Z_{i,t}\right) \times SM_{i,t-1} \times bank.dep_{i}  \times bond_{i}$ & &
% & & & & & -- \\ \addlinespace[5pt]

% $ NZ_{i,t-1} \times \Delta log\left(BN^Z_{i,t}\right) \times SM_{i,t-1} \times bank.dep_{i} \times no.bond_{i}$ & & 
% & & & & & -- \\ \addlinespace[5pt]
 
% $ NZ_{i,t-1} \times \Delta log\left(BN^Z_{i,t}\right) \times SM_{i,t-1} \times bank.dep_{i} \times bond_{i}$ & & 
% & & & & & -- \\ \addlinespace[5pt]
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 
\addlinespace[10pt]

Years & & 2002-2020 & 2002-2020 & 2002-2020\\ 
Observations & & 43,848 & 27,326 & 27,326 \\ 
Firms & & 7,444 & 3,874 & 3,874 \\   
Fixed Effects & & X &  X & X \\
Controls & & X &  X & X \\
Within-$R^2$ & & 0.06 & 0.07 & 0.07 \\   


\hline
\addlinespace[1pt]
\end{tabular}
\end{center}
\noindent \tiny Notes: For better visualization, coefficients are multiplied by a factor of $10^2$. Each estimation includes firm-, industry-, year- and -industry-year-fixed effects. Standard errors are clustered at the firm-level.
%We restrict the sample to only those companies that reported either one of the bank-credit instruments, $BL$ or $RC$, or an issuance of \textit{bonds \& notes} (BN) at least once over the period 2002 - 2019. For these variables -- and those interacted with the non-zombie-indicator ($ BC^{Z}_{i,t}, BN^{Z}_{i,t} $). 
Controls include a lagged measure of size ($log\left(AT_{i,t-1}\right)$), a firm's lagged cash ratio ($CHE_{i,t-1} / LT_{i,t-1}$), it's profitability ($ROA_{i,t-1} = IB_{i,t-1} / AT_{i,t-1}$),and the lagged proxy for a firm's asset tangibility ($PPENT_{i,t-1} / AT_{i,t-1}$). Robust standard errors in parentheses: *** p$<$0.01, ** p$<$0.05, * p$<$0.1 \\
\end{table}

==> 10_Estimation/Model00_oldEMP.tex <==
\begin{table}[H]
%\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.75}
    \begin{center}
    %\vspace{-2cm}
    \captionsetup{justification=centering}
    \footnotesize
\caption{\label{tab:Model00_Z_v3} Regressions Results: Zombie-Lending \& Non-Zombie Performance \\ Zombie-Definition $Z^{NAR}$}
 

\begin{tabular}{l cccc} \hline
\addlinespace[2pt]
 Maturity ($m$) & & 1Q  $\leq m \leq$ 4Q & 1Q  $\leq m \leq$ 4Q 
 & 1Q  $\leq m \leq$ 4Q \\ 
 \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
 & & (1)  & (2) & (3)  \\
Variables & & $TFP_{i,t}$ & $\Delta log \left(K_{i,t}\right)$ & 
$\Delta EMP_{i,t}$  \\  \addlinespace[2pt] \hline

\addlinespace[10pt]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$ NZ_{i,t-1} $ & &
 -0.010 & 0.196*** & 7.907*** \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addlinespace[5pt]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$ NZ_{i,t-1} \times BC^Z_{s,t-1}$ & &
-0.100 & -0.257 & \\ \addlinespace[5pt]

$ NZ_{i,t-1} \times BN^Z_{s,t-1} $& & 
0.202 & 0.091 & \\ \addlinespace[5pt]

$ NZ_{i,t-1} \times \Delta log \left(BC^Z_{s,t}\right)$ & &
 & & -0.293 \\ \addlinespace[5pt]

$ NZ_{i,t-1} \times \Delta log \left( BN^Z_{s,t}\right) $& & 
 &  & -0.220 \\ \addlinespace[5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addlinespace[10pt]

Years & & \multicolumn{3}{c}{2002 - 2020} \\ 
Observations & & 41,098 & 72,381 & 43,848 \\ 
Firms & & 5,826 & 9,709 & 7,444 \\   
Fixed Effects & & X &  X & X \\
Controls & & X &  X & X \\
Within-$R^2$ & & 0.03 & 0.12 & 0.05 \\   

\addlinespace[5pt]
    \midrule
\addlinespace[5pt]

Maturity ($m$) & & 5Q  $\leq m \leq$ 40Q & 5Q  $\leq m \leq$ 40Q 
 & 5Q  $\leq m \leq$ 40Q \\ 
 \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
 & & (4)  & (5) & (6)  \\
Variables & & $TFP_{i,t}$ & $\Delta log \left(K_{i,t}\right)$ & 
$\Delta EMP_{i,t}$  \\  \addlinespace[2pt] \hline

\addlinespace[10pt]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$ NZ_{i,t-1} $ & &
 -0.006 & 0.192-*** & 7.638*** \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addlinespace[5pt]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$ NZ_{i,t-1} \times BC^Z_{s,t-1}$ & &
-0.476 & -0.407 &  \\ \addlinespace[5pt]

$ NZ_{i,t-1} \times BN^Z_{s,t-1} $& & 
-0.039 & 0.446 &  \\ \addlinespace[5pt]

$ NZ_{i,t-1} \times \Delta log \left(BC^Z_{s,t}\right)$ & &
 &  & -0.487 \\ \addlinespace[5pt]

$ NZ_{i,t-1} \times \Delta log \left(BN^Z_{s,t}\right) $& & 
 &  & -0.624 \\ \addlinespace[5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addlinespace[10pt]

Years & & \multicolumn{3}{c}{2002 - 2020} \\ 
Observations & & 41,100 & 72,466 & 55,607 \\ 
Firms & & 5,827 & 9,713 & 8,503 \\   
Fixed Effects & & X &  X & X \\
Controls & & X &  X & X \\
Within-$R^2$ & & 0.03 & 0.12 & 0.06 \\  

\hline
\addlinespace[1pt]
\end{tabular}
\end{center}
\noindent \tiny Notes: Each estimation includes firm-, industry-, year- and -industry-year-fixed effects. Standard errors are clustered at the firm-level.
% We restrict the sample to only those companies that reported either one of the bank-credit instruments, $BL$ or $RC$, or an issuance of \textit{bonds \& notes} (BN) at least once over the period 2002 - 2019. For these variables -- and those interacted with the non-zombie-indicator ($ BC^{Z}_{i,t}, BN^{Z}_{i,t} $). 
Controls are composed as follows: Models (1) and  (4) include a lagged measure of size ($log\left(AT_{i,t-1}\right)$) and a firm's lagged R\&D intensity ($XRD_{i,t-1} / AT_{i,t-1}$). 
Models (2) and  (5) include a lagged measure of size ($log\left(AT_{i,t-1}\right)$) and a firm's lagged asset tangibility ($PPENT_{i,t-1} / AT_{i,t-1}$)
Models (3) and  (6) include a lagged measure of size ($log\left(AT_{i,t-1}\right)$), a firm's lagged cash ratio ($CHE_{i,t-1} / LT_{i,t-1}$), it's profitability ($ROA_{i,t-1} = IB_{i,t-1} / AT_{i,t-1}$),and the lagged proxy for a firm's asset tangibility ($PPENT_{i,t-1} / AT_{i,t-1}$).
For better visualization, coefficients for Models (3) and (6) are multiplied by a factor of $10^2$.
Robust standard errors in parentheses: *** p$<$0.01, ** p$<$0.05, * p$<$0.1\\
\end{table}

==> 10_Estimation/NewbiesEMPgr_Z_v3_oldEMP.tex <==
\begin{table}[h!]
    \begin{center}
    \captionsetup{justification=centering}
    \footnotesize
\caption{\label{tab:NewbiesEMPgr_Z_v3} Regressions Results: Newbies, Employment Growth \& Zombie-Lending -- Zombie-Definition $Z^{NAR}$}
 

\begin{tabular}{l ccccc} \hline
 \addlinespace[2pt]
 Maturity ($m$) & & 1Q  $\leq m \leq$ 4Q & 5Q  $\leq m \leq$ 40Q & 1Q  $\leq m \leq$ 4Q & 5Q  $\leq m \leq$ 40Q 
\\
 \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}
 & & (1) & (2) & (3) & (4) \\
Variables & & $\Delta EMP_{i,t}$ & $\Delta EMP_{i,t}$ & $\Delta log \left(EMP_{i,t}\right)$ & $\Delta log \left(EMP_{i,t}\right)$  \\  \addlinespace[2pt] \hline


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$ NB_{i,t-1} $ & &
0.061*** &  0.051*** & 
0.073*** & 0.054*** \\ \addlinespace[5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addlinespace[10pt]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$ NB_{i,t-1} \times \Delta log\left(BC^Z_{s,t}\right) $ & &
-0.007 &  -0.001  & 
-0.011 & 0.006 \\ \addlinespace[5pt]

$ NB_{i,t-1} \times \Delta log\left(BN^Z_{s,t}\right) $ & & 
-0.003 &  -0.011*  & 
-0.002 & -0.013 \\ \addlinespace[5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\addlinespace[10pt]

Years & & 2002-2020 & 2002-2020 & 2002-2020 & 2002-2020\\ 
Observations & & 44,073 & 56,493 & 44,073 & 56,493 \\ 
Firms & & 7,177 & 8,229 & 7,177 & 8,229 \\   
Fixed Effects & & X & X & X & X \\
Controls & & X &  X&  X & X \\
Within-$R^2$ & & 0.12 & 0.13 & 0.11 & 0.12 \\ 

\hline
\addlinespace[1pt]
\end{tabular}
\end{center}
\noindent \scriptsize Notes: Each estimation includes firm-, sector-, year- and sector-year-fixed effects. Standard errors are clustered at the firm-level. 
%We restrict the sample to only those companies that reported either one of the bank-credit instruments, $BL$ or $RC$, or an issuance of \textit{bonds \& notes} (BN) at least once over the period 2002 - 2019. For these variables -- and those interacted with the non-zombie-indicator ($ BC^{Z}_{i,t}, BN^{Z}_{i,t} $).
Control variables are lagged and include a proxy for firm size ($log\left(AT_{i,t-1}\right)$),  a firm's asset tangibility, i.e. the capital-to-asset ratio ($PPENT_{i,t-1} / AT_{i,t-1}$), and the first-difference of $log\left( SALE_{i,t}\right)$. Robust standard errors in parentheses: *** p$<$0.01, ** p$<$0.05, * p$<$0.1 \\ %as a proxy for business opportunities \citep{CaballeroHoshiKashyap2008,McGowanAndrewsMillot2018}. \\
\end{table}
